CASH: A Credit Aware Scheduling for Public Cloud Platforms

The public cloud offers a myriad of services which allows its tenants to process large scale big data in a flexible, easy and cost effective manner. Tenants generally use large scale data processing frameworks such as MapReduce, Tez, Spark etc. to process their data. Tenants can configure their frameworks to run individual tasks by the framework itself or have a middleware cluster manager like YARN or Mesos to arbitrate resource scheduling in their public-cloud cluster. Cluster managers need to be cognizant about the workload requirement along with the state of the individual resource such as CPU and disk in the cluster. Cloud providers use a token bucket mechanism for their individual hardware resources as an indicator of the quality-of-service that individual hardware resource can provide. In this paper, through our changes in YARN, Hadoop and Tez, we show how middleware cluster managers can be made cognizant about the expected quality-of-service of individual hardware resources in the cluster. Our optimized cluster manager with a coarse grained knowledge of task requirement and fine grained knowledge of expected quality-of-service of hardware resources in the cluster performs highly optimal task placements. Our experiments with our optimizations show CPU credit based instances like the Amazon T3 instances as a viable cost effective option for running bigdata workloads. We also show that streaming SQL queries on a Hive warehouse can be accelerated by up to 31% leading to public cloud cost savings of up to 22%.

==> authors.tex <==
% \begin{comment}

% \author{
% \centering
% \IEEEauthorblockN{ Aakash Sharma}
% \IEEEauthorblockA{\textit{Dept. of Electrical Engineering and Computer Science} \\
% \textit{Pennsylvania State University}\\
% University Park, PA \\
% abs5688@psu.edu}\\
% %\and
% \centering
% \IEEEauthorblockN{Saravanan Dhakshinamurthy}
% \IEEEauthorblockA{
% \textit{Facebook, Inc.}\\
% Menlo Park, CA \\
% saravanand@fb.com}\\
% %\and
% \centering
% \IEEEauthorblockN{Chita R. Das}
% \IEEEauthorblockA{\textit{Dept. of Electrical Engineering and Computer Science} \\
% \textit{Pennsylvania State University}\\
% University Park, PA \\
% cxd12@psu.edu}\\
% %\and
% \centering
% \IEEEauthorblockN{George Kesidis}
% \IEEEauthorblockA{\textit{Dept. of Electrical Engineering and Computer Science} \\
% \textit{Pennsylvania State University}\\
% University Park, PA \\
% gik2@psu.edu}\
% }
% \end{comment}


 \author{
    \IEEEauthorblockN{
     Aakash Sharma\IEEEauthorrefmark{1},
     Saravanan Dhakshinamurthy\IEEEauthorrefmark{2},
     George Kesidis\IEEEauthorrefmark{1},
     Chita R. Das\IEEEauthorrefmark{1},
     }

    \IEEEauthorblockA{
     \IEEEauthorrefmark{1}The Pennsylvania State University, University Park \IEEEauthorrefmark{2} Facebook Inc. \vspace{2mm}
     }
}

==> redundent.tex <==
% @online{Hadoop_at_Facebook,
%   author = {Facebook},
%   title = {Hadoop},
%   year = 2008,
%   url = {https://www.facebook.com/notes/facebook-engineering/hadoop/16121578919/},
%   urldate = {2008-06-05}
% }

% @inproceedings{hasanIOAWS,
% author = {Nawaz, Hassan and Juve, Gideon and Ferreira da Silva, Rafael and Deelman, Ewa},
% year = {2016},
% month = {05},
% pages = {535-544},
% title = {Performance Analysis of an I/O-Intensive Workflow Executing on Google Cloud and Amazon Web Services},
% doi = {10.1109/IPDPSW.2016.90}
%}




% @inproceedings{DBLP:conf/sosp/GhemawatGL03,
%   author    = {Sanjay Ghemawat and
%               Howard Gobioff and
%               Shun{-}Tak Leung},
%   title     = {The Google file system},
%   booktitle = {Proceedings of the 19th {ACM} Symposium on Operating Systems Principles
%               2003, {SOSP} 2003, Bolton Landing, NY, USA, October 19-22, 2003},
%   pages     = {29--43},
  
%   }




\begin{itemize}
\item Hadoop MapReduce Project
\item Hadoop YARN Project
\item Hadoop HDFS project
\end{itemize}

\subsubsection{Hadoop MapReduce Project}
Hadoop is an open source java based implementation of MapReduce which is the dominant big data processing framework of today's time. The Hadoop Mapreduce project is the data processing layer of Hadoop. It contains the Application Master(AM), mappers and reducers which collectively process user data based on the application logic. The AM is responsible for negotiating resources with the cluster manager and executing mappers and reducers on those resources. The AM forms the schedule of tasks to be executed in the cluster and submits resource request to the cluster manager to execute them.
\\
\subsubsection{Hadoop HDFS Project}
HDFS stands for Hadoop Distributed File System. Although no longer exclusively used by Hadoop, HDFS is widely used as an open source distributed network based file system which supports large block sizes for high sequential read/write throughput. It also provides replication while running on commodity hard disks. HDFS exposes the entire storage infrastructure of the cluster as one large file system which applications can use to store and share data. Multiple frameworks and applications running together on a cluster use HDFS to store data which can then be used across the whole cluster. HDFS model is inspired by the Google file system\cite{DBLP:conf/sosp/GhemawatGL03}
\\
\subsubsection{Hadoop YARN Project}
YARN is the job scheduler and resource manager used by Hadoop. YARN is also a cluster manager on its own and it can be used to manage the entire resources of a cluster with multiple frameworks and users sharing the cluster at the same time. YARN can also be used to run "standalone" applications, wherein the application simply requests for resources from YARN and executes its tasks. Hadoop in particular is tightly integrated with YARN and lacks a scheduler of its own.\\
YARN uses a priority based random scheduling within the same job wherein tasks of the same job are executed within YARN containers in the priority order specified by the job and randomly within the same priority. YARN itself has two schedulers, the capacity scheduler and the fair scheduler. Capacity scheduler supports various hierarchical queues to which jobs can be submitted. The highest level queue or the "root" queue has access to 100\% of the capacity of the cluster. The root queue can have multiple child queues which in turn can have multiple child queues. A queue at each level can have a capacity between 0 - 100\% of its parent queue. Each queue have a access control list allowing a certain subset of users to submit jobs to it and finally queues can be tagged with labels to allow only certain jobs to be run on them. All in all, capacity scheduler provides good resource isolation when many users and their jobs are competing for the cluster resources. Scheduling within a queue can be FIFO or fair. On the other hand the fair scheduler provides fair scheduling for a particular job's tasks. At the time of writing this paper, we have found no evidence of one scheduler being better then the other.
The basic architecture, components of Hadoop is explained in Figure 2.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Main/images/Hadoop_architecture.png}
    \caption{Hadoop Components}
    \label{fig:hadoopComponents}
\end{figure}



Hadoop workloads comprise a number of jobs which are subdivided into a number of tasks. Hadoop tasks are either map tasks or reduce tasks. Map tasks work on a certain part of input data, performing operations on them. The output data from all map tasks are then "shuffled" via the network as input to reduce tasks. The reduce tasks sorts the input data from mappers and collates them to produce the final output.\par
Tasks are extremely I/O intensive as Hadoop constantly read/writes from storage to accommodate the large data it is processing. The nature of input data is such that it can never completely fit in memory and data is "spilled" on to storage. However, when Hadoop does have data available in memory after reading from storage, its tasks become CPU intensive. Hence, Hadoop comprise a set of I/O intensive and CPU intensive tasks.\par



MapReduce is a key recipe in any large scale data processing cluster. It is essentially the first large scale data processing framework made for the internet scale by Google. Google used MapReduce in its initial days to process the internet scale web pages to power its search engine. Upon the release of Google's MapReduce paper in 2004, a lot of interest was generated in MapReduce. Yahoo then came out with the open source implementation of MapReduce with Hadoop. Hadoop quickly became the quintessential big data processing framework across the industry. Facebook has been one of the early users of Hadoop, going back to 2008 when it was loading over 2 TBs of data into Hadoop everyday\cite{Hadoop_at_Facebook}.\par
Hadoop MapReduce framework comes prepackaged with Apache YARN\cite{yarn} resource scheduler. YARN is an event based scheduler which can be used as a resource scheduler and a cluster manager to run Hadoop, Spark and other data processing frameworks. Any process can ask for resource from YARN by submitting jobs to it. YARN allocates cluster resources in the form of containers having fixed CPU cores and memory for good resource isolation. Default container in YARN are java containers but it can be configured to use Linux cgroups\cite{cgroup} or even docker\cite{docker}.\\
MapReduce is the basic parallel data processing framework for big data. This model was created by Google to run their pagerank algorithm and other data processing jobs in the cluster.



Hadoop requires two different kinds of storage to run its workloads. The input and output of individual jobs need to be stored in a distributed highly available file system which also supports replicas like HDFS. This allows Hadoop jobs to be highly resilient to node failures as data stored in an individual node is always replicated and can be accessed from anywhere over the network. On node failure or even in case of a straggling job, Hadoop can always reschedule the job in some other node allowing high resilience in job execution. However, the intermediate data which is generated by individual tasks such as the output of a map task before being shuffled to a reducer is stored on a local file system. This intermediate data need not be highly available and is at best temporary in nature. Particularly nodes where reducer tasks are executed need a high amount of this temporary storage as they shuffle the output of all map tasks to be collated by them.


AWS instance storage (DAS) is mostly small and is not suitable for processing large amount of data needed for today's big data workloads. Only certain type of instances, like storage optimized (h1 and i3) have large instance storage for storing big data workloads and they have high pricing. This leaves the user to use either EBS or S3 for storage.\\
Both EBS and S3 are network attached storage which are highly available through SLA guarantees from Amazon and hence individual file blocks/buckets do not need any replication. Since these stores are network attached, there is always a network transfer latency incurred, unlike DAS. AWS users have a preference to have S3 as their data store. As described in the introduction, users run Hadoop on AWS because they have data on S3 through some other service. Downloading data from S3 to private data center is billed by AWS. S3 is also the most cost effective storage option offered by AWS. Table 4 describes the various storage options which can be used for data processing that AWS provides and their pricing. S3 charges additionally for all S3 requests from within AWS and data transfer to external world and external AWS region. The S3 request pricing (per 1000 requests) can be found in table 5 and data transfer out from S3 to internet pricing in table 6. All pricing mentioned is for S3 standard.
\input{Main/Tables/aws_storage_price.tex} 
\input{Main/Tables/s3ReqPrice.tex}
\input{Main/Tables/s3DataTransferPrice.tex} 



However, the rise in performance of storage technology in the last 5 years has contributed to higher CPU utilization in data processing cluster. EBS storage provide high throughput (up to 150 Mbps) and Hadoop does provide high CPU utilization as confirmed by our experiments in the next section. But Hadoop must also read and write to S3 which degrades CPU utilization. T3.2xlarge instances provide a baseline performance of 40\% and a ability to burst with accumulated credits. If the average CPU utilization of a workload remains low, T3 can provide excellent cost savings.\\


Having input data on S3 and writing output of a job back to S3 completely eliminates the need of having a distributed file system like HDFS. Amazon EMR provides EMRFS as an alternative to HDFS which is essentially a connector to S3. Apache has their own open source S3 connector called s3a. 



\begin{itemize}
    \item I/O bound
    \item CPU bound
    \item Mixed
\end{itemize}

We then recommend the tenant to follow the following order:
\begin{enumerate}
\item I/O bound jobs
\item Mixed jobs
\item CPU bound jobs
\end{enumerate}
Following this order allows T3 instances to accumulate credit for future expenses. I/O bound jobs spend a lot of time with low CPU utilization doing I/O over S3. On the other hand CPU bound jobs spend little time doing I/O with S3 and as a result they have very high CPU utilization. Running I/O bound jobs before CPU bound allows credits to be accumulated which is then used by CPU bound jobs. Mixed job can be run in any order if they have an average CPU utilization at or below the baseline of T3 instance type. We gather most MapReduce workloads operate with average CPU utilization at or below the t3.2xlarge baseline of 40\%. \par


A key observation to note here is that a T3.2xlarge instance operating at an average CPU utilization of 52.5\% will be billed as much as an equivalent M5 general purpose instance and an instance operating at 100\% CPU utilization will be billed close to 50\% more than an equivalent M5 general purpose instance, wiping out any cost savings of using burstable instances.

Tenants running workloads on EMR can find the average CPU utilization of their workloads through EMR itself. EMR provides excellent monitoring features, allowing its users to easily discern the CPU utilization of their workloads. Tenants of EMR may decide to use T3 if they observe a low CPU utilization in their workloads. We propose a combination of following two schemes to deliver maximum cost savings with the lowest makespan.

Since YARN follows random scheduling while choosing nodes to schedule tasks, a task may be assigned on a 0 CPU credit node while there are available nodes with available CPU credit balance. This makes the task a straggler. Stragglers have the ability to completely remove any improvement in job completion time and wipe out cost savings. Alternatively, a tenant running T3 unlimited will be billed extra for an instance with 0 credits while there are still instances available with remaining credits. On the other hand, YARN may allocate multiple reducers on a single node. This brings down the CPU utilization of a node and reducers being long running tasks with high memory footprint, will make the host node accumulate too many credits. These credits are accumulated while other CPU bound map tasks are running on nodes with low or 0 CPU credit balance, slowing down the job completion time along with other problems discussed in the next section.\\
To avoid both these problems, we introduce our second optimization.

==> results.tex <==
\section{Results}




